Deep Generative Models that Solve PDEs: Distributed Computing for Training Large Data-Free Models

Recent progress in scientific machine learning (SciML) has opened up the possibility of training novel neural network architectures that solve complex partial differential equations (PDEs). Several (nearly data free) approaches have been recently reported that successfully solve PDEs, with examples including deep feed forward networks, generative networks, and deep encoder-decoder networks. However, practical adoption of these approaches is limited by the difficulty in training these models, especially to make predictions at large output resolutions ($\geq 1024 \times 1024$). Here we report on a software framework for data parallel distributed deep learning that resolves the twin challenges of training these large SciML models - training in reasonable time as well as distributing the storage requirements. Our framework provides several out of the box functionality including (a) loss integrity independent of number of processes, (b) synchronized batch normalization, and (c) distributed higher-order optimization methods. We show excellent scalability of this framework on both cloud as well as HPC clusters, and report on the interplay between bandwidth, network topology and bare metal vs cloud. We deploy this approach to train generative models of sizes hitherto not possible, showing that neural PDE solvers can be viably trained for practical applications. We also demonstrate that distributed higher-order optimization methods are $2-3\times$ faster than stochastic gradient-based methods and provide minimal convergence drift with higher batch-size.

==> MatrixAssemblyData.tex <==
\begin{figure}[h]
\centering
\begin{tikzpicture}[
  every axis/.style={
    ybar stacked,
    ymin=0,ymax=17,
    ylabel = Time (in s),
    x tick label style={
       % add some negative yshift to move ticklabels down
       yshift=-4mm,
       rotate=45,
       anchor=east},
%   x axis line style = { opacity = 0 }, 
%   y axis line style = { opacity = 0 },
  tickwidth = 0pt,
  legend style={
    legend columns=2,
        yshift=0mm,
        xshift = -40 mm,
        anchor=north,
        draw=none
    },
%   width=15cm,
%   height=8cm,
  % symbolic coords have numerical distance of 1
  % so with the following line you get a tick at every symbolic coord
  xtick distance=1,
  symbolic x coords={
      Skx Stampede,
      SkyLake Frontera,
      KNL stampede,
    },
  bar width=6pt
  },
]

\pgfplotsset{
  % define a new style used for the plot used to add labels
  % 2 args means it takes two mandatory arguments, so must be used as
  % labelplot={first arg}{second arg}
  labelplot/.style 2 args={
     % forget plot means it doesn't affect cycle lists or legends
     forget plot,
     % #1 is first argument, the text used in the nodes near coords
     nodes near coords=#1,
     % #2 is second argument, a length that should be the same as the bar shift for the axis
     every node near coord/.style={below,font=\tiny,xshift=#2}
  }
}
% Without Tensor
\begin{axis}[bar shift=-12pt, xticklabels={}]
\addplot [labelplot={GP}{-12pt}] coordinates
{(Skx Stampede,0) (SkyLake Frontera,0) (KNL stampede,0)};
\addplot coordinates
{(Skx Stampede,1.0617e+00) (SkyLake Frontera,8.0538e-01) (KNL stampede,5.4996e+00)};
\addplot coordinates
{(Skx Stampede,3.1981) (SkyLake Frontera,2.33232) (KNL stampede,9.5344)};
\end{axis}

\begin{axis}
\addplot [labelplot={MM}{0pt}] coordinates
{(Skx Stampede,0) (SkyLake Frontera,0) (KNL stampede,0)};
\addplot coordinates
{(Skx Stampede,7.7540e-01) (SkyLake Frontera,5.6241e-01) (KNL stampede,3.7750e+00)};
\addplot coordinates
{(Skx Stampede,3.1447) (SkyLake Frontera,2.56089) (KNL stampede,9.616 )};
\legend{Assembly time, Total solve time}
\end{axis}
\end{tikzpicture}
 \caption{Comparison of time on different cluster for matrix assembly and complete solve time for linear basis function.}
 \label{fig:MatAssemblyLinear}
\end{figure}

\begin{figure}
\begin{tikzpicture}[
  every axis/.style={
    ybar stacked,
    ymin=0,ymax=700,
    ylabel = Time (in s),
    x tick label style={
       % add some negative yshift to move ticklabels down
       yshift=-4mm,
       rotate=45,
       anchor=east},
        legend style={
    legend columns=2,
        yshift=0mm,
        xshift = -40 mm,
        anchor=north,
        draw=none
    },
%   x axis line style = { opacity = 0 }, 
%   y axis line style = { opacity = 0 },
  tickwidth = 0pt,
%   width=15cm,
%   height=8cm,
  % symbolic coords have numerical distance of 1
  % so with the following line you get a tick at every symbolic coord
  xtick distance=1,
  symbolic x coords={
      Skx Stampede,
      SkyLake Frontera,
      KNL stampede,
    },
  bar width=6pt
  },
]

\pgfplotsset{
  % define a new style used for the plot used to add labels
  % 2 args means it takes two mandatory arguments, so must be used as
  % labelplot={first arg}{second arg}
  labelplot/.style 2 args={
     % forget plot means it doesn't affect cycle lists or legends
     forget plot,
     % #1 is first argument, the text used in the nodes near coords
     nodes near coords=#1,
     % #2 is second argument, a length that should be the same as the bar shift for the axis
     every node near coord/.style={below,font=\tiny,xshift=#2}
  }
}
\begin{axis}[bar shift=-12pt, xticklabels={}]
\addplot [labelplot={GP}{-12pt}] coordinates
{(Skx Stampede,0) (SkyLake Frontera,0) (KNL stampede,0)};
\addplot coordinates
{(Skx Stampede,7.1132e+01) (SkyLake Frontera,5.9356e+01) (KNL stampede,3.8559e+02)};
\addplot coordinates
{(Skx Stampede,163.078) (SkyLake Frontera,153.414) (KNL stampede,278.46)};
\end{axis}

\begin{axis}
\addplot [labelplot={MM}{0pt}] coordinates
{(Skx Stampede,0) (SkyLake Frontera,0) (KNL stampede,0)};
\addplot coordinates
{(Skx Stampede,1.0245e+01) (SkyLake Frontera,8.4647e+00) (KNL stampede,4.0409e+01)};
\addplot coordinates
{(Skx Stampede,164.785) (SkyLake Frontera,155.9953) (KNL stampede,305.741 )};
\legend{Assembly time, Total solve time}
\end{axis}
\end{tikzpicture}
 \caption{Comparison of time on different cluster for matrix assembly and complete solve time for quadratic basis function. GP indicates the assembly over looping over the individual Gauss points and MM indicates the assembly by imposing FEM operator as matrix - matrix multiplication.}
 \label{fig:MatAssemblyQuad}
\end{figure}


